ShapeNet: Shape Constraint for Galaxy Image Deconvolution

Deep Learning (DL) has shown remarkable results in solving inverse problems in various domains. In particular, the Tikhonet approach is very powerful to deconvolve optical astronomical images (Sureau et al. 2020). Yet, this approach only uses the $\ell_2$ loss, which does not guarantee the preservation of physical information (e.g. flux and shape) of the object reconstructed in the image. In Nammour et al. (2021), a new loss function was proposed in the framework of sparse deconvolution, which better preserves the shape of galaxies and reduces the pixel error. In this paper, we extend Tikhonet to take into account this shape constraint, and apply our new DL method, called ShapeNet, to optical and radio-interferometry simulated data set. The originality of the paper relies on i) the shape constraint we use in the neural network framework, ii) the application of deep learning to radio-interferometry image deconvolution for the first time, and iii) the generation of a simulated radio data set that we make available for the community. A range of examples illustrates the results.

==> ellipticity.tex <==
The shape information of galaxies is essential in various fields of astrophysics, such as Galaxy Evolution and Cosmology. The measure that is used to study the shape of a galaxy is the ellipticity, which is a complex scalar, $e = e_1 + \bold{i} e_2$. By noting $x\in\mathbb{R}^{n \times n}$ the galaxy image, its ellipticity is given by \citep{kaiser1995ksb}:
\begin{equation}
    e(x) = \frac{\mu_{2,0}(x)-\mu_{0,2}(x) + \bold{i} 2\mu_{1,1}(x)}{\mu_{2,0}(x)+\mu_{0,2}(x)} \quad,
\end{equation}
where $\mu_{s,t}$ are the image centered moments of order $(s+t)$ defined as:
\begin{equation}
    \mu_{s,t}(x) = \sum_{i=1}^n \sum_{j=1}^n x\left[(i-1)n+j\right]\left(i-i_c\right)^s\left(j-j_c\right)^t \quad,
\end{equation}
and $i_c$ and $j_c$ are the coordinated of the centroid of $x$, such that:
\begin{equation}
    i_c = \frac{\sum_{i=1}^n \sum_{j=1}^n i\cdot x\left[(i-1)n+j\right]}{\sum_{i=1}^n \sum_{j=1}^n x\left[(i-1)n+j\right]}
\end{equation}
and
\begin{equation}
    j_c = \frac{\sum_{i=1}^n \sum_{j=1}^n j\cdot x\left[(i-1)n+j\right]}{\sum_{i=1}^n \sum_{j=1}^n x\left[(i-1)n+j\right]} \quad.
\end{equation}
A direct way of formulating a shape constraint would be adding a data-fidelity term in the ellipticity space. However the measure $e(x)$ is not linear regarding $x$, which complicates the study of its property such as its gradient and the noise propagation. For this purpose, we derived the following reformulation in \cite{nammour2021galaxy}:
\begin{equation}
    \label{eq:e1_scal}
    e_1 = \frac{\left<x,u_3\right>\left<x,u_4\right>-\left<x,u_1\right>^2+\left<x,u_2\right>^2}{\left<x,u_3\right>\left<x,u_4\right>-\left<x,u_1\right>^2-\left<x,u_2\right>^2}
\end{equation}
and
\begin{equation}
    \label{eq:e2_scal}
    e_2 = \frac{2\left(\left<x,u_3\right>\left<x,u_6\right>-\left<x,u_1\right>\left<x,u_2\right>\right)}{\left<x,u_3\right>\left<x,u_4\right>-\left<x,u_1\right>^2-\left<x,u_2\right>^2} \quad,
\end{equation}
where $\left\{u_1,\dots,u_6\right\} \in\mathbb{R}^{6 \times n \times n}$ are constant images defined, for all $i$, $j$ in $\{1,\cdots, n\}$, as:
\begin{equation}
    \begin{aligned}
        &u_1[(i-1)n+j] = i, &&u_2[(i-1)n+j] = j,\\
        &u_3[(i-1)n+j] = 1, &&u_4[(i-1)n+j] = (i^2+j^2),\\
        &u_5[(i-1)n+j] = (i^2-j^2), &&u_6[(i-1)n+j] = (ij).
    \end{aligned}
\end{equation}
All the scalar products in eq. \ref{eq:e1_scal} and \ref{eq:e2_scal} are linear regarding $x$. Therefore, by formulating the shape constraint as a data-fidelity term in these scalar products space, we obtain:
\begin{equation}
    \label{eq:shape_constraint_nowin}
    M_0(x) = \sum_{i=1}^6 \omega_i \left<h \ast x - y, u_i\right>^2 \quad,
\end{equation}
where $\left\{\omega_1,\dots,\omega_6\right\}$ are non-negative scalar weights. These weights are set by considering the noise propagation as argued in \cite{nammour2021galaxy}. Eq. \ref{eq:shape_constraint_nowin} offers a shape constraint which properties are straightforwardly derived. However the ellipticity measure is extremely sensitive regarding noise. To add robustness to the shape constraint, we considered windowing the observed image, $y$, to reduce the noise effect. One approach is to fit a Gaussian window on $y$, however it would require an additional preprocessing step on each observed image. To avoid this step, we chose to use a set of precomputed windows such that at least one of them fits the galaxy in the observed image. We considered curvelets to look for a candidate set, since they are a family of linear multi-scale transforms that are usually designed with specific properties to efficiently represent objects of interest. This lead us to eq. \ref{eq:shape_constraint}.

==> sota.tex <==
%In the following we give the state of the art methods to image restoration in both optical and radio imaging.
%
\subsection{Sparse restoration}
\label{subsec:sparsity}

Sparsity is a powerful regularization to solve inverse problems, in particular deconvolution \citep{donoho1995wavelet,starck2015sparse,farrens2017}. Using it on astrophysical images requires a suited transform that offers a sparse representation of the galaxy signal, it is the case of the Starlet transform as shown in \citep{starck2015sparse}. Various methods based on sparsity have been proposed in both radio \citep{carin2009radioCS,wiaux2009radio,carrillo2012sara,carrillo2014purify,garsden2015} and optical imaging \citep{nammour2021galaxy,farrens2017} such as the \acrfull{SRA} and \acrfull{SCORE}. The two methods use a Forward Backward Splitting frame to reconstruct the galaxy image by minimising a loss function. The function contains in both cases a data-fidelity term, a positivity constraint, a sparsity constraint using the starlet transform and in the case of \acrshort{SCORE} an additional shape constraint term detailed in \ref{subsec:shape_constraint}.

\subsection{Deep Learning}
\label{subsec:deep_learning}
In recent years, the emergence of \acrfull{DL} has shown promising results in various domains, including deconvolution \citep{xu2014dcnn}. In astrophysics, methods based on \acrshort{DL} have already been developed to perform model fitting which can be seen as parametric deconvolution \citep{tuccillo2018deepfitting}. In contrast to sparse reconstruction methods, there are fewer priors on the reconstruction in the case of \acrshort{DL} which reduces the expected model bias, we can cite the Tikhonet developed by \cite{sureau2020}.%(see \ref{subsec:tikho}) developed by \cite{sureau2020}.

\subsection{CLEAN}
\label{subsec:clean}
Along with \acrfull{MEM}~\citep{cornwell1985mem,chen2021rem}, CLEAN~\citep{hogbom1974aperture} is a standard deconvolution algorithm in radio imaging. The core idea of this algorithm is to extract a list of the maxima that are three times higher than the standard deviation of the values in the observed image, also called \emph{dirty image}. A smooth convolution kernel (a two-dimensional Gaussian usually), called \emph{CLEAN beam}, is fitted on the \acrshort{PSF}, called \emph{dirty beam}. The list of maxima is then convolved with the CLEAN beam to obtain the reconstructed image, called \emph{CLEAN image}. CLEAN is a fast iterative and non-linear method, its reconstruction of extended sources is problematic. Many ameliorations have been suggested, namely by \cite{clark1980efficient,schwab1984relaxing}. A popular variant of CLEAN, called CLEAN isotropic, uses an isotropic Gaussian PSF with a standard deviation $\sigma$ equal to 2 pixels and a flux normalized by that of the CLEAN beam. This convolution makes it possible to soften the map of the detected CLEAN components composed exclusively of diracs, and to adapt their representation to the fact that the ground truth galaxy is extensive. 

All of the sparse, \acrshort{DL} and CLEAN methods do not offer any guarantee on the shape conservation in the reconstructed image.
